How Do Developers Structure Unit Test Cases? An Empirical Study from the "AAA" Perspective

The AAA pattern, i.e. arrange, act, and assert, provides a unified structure for unit test cases, which benefits comprehension and maintenance. However, there is little understanding regarding whether and how common real-life developers structure unit test cases following AAA in practice. In particular, are there recurring anti-patterns that deviate from the AAA structure and merit refactoring? And, if test cases follow the AAA structure, could they contain design flaws in the A blocks? If we propose refactoring to fix the design of test cases following the AAA, how do developers receive the proposals? Do they favor refactoring? If not, what are their considerations? This study presents an empirical study on 435 real-life unit test cases randomly selected from four open-source projects. Overall, the majority (71.5%) of test cases follow the AAA structure. And, we observed three recurring anti-patterns that deviate from the AAA structure, as well as four design flaws that may reside inside of the A blocks. Each issue type has its drawbacks and merits corresponding refactoring resolutions. We sent a total of 18 refactoring proposals as issue tickets for fixing these problems. We received 78% positive feedback favoring the refactoring. From the rejections, we learned that return-on-investment is a key consideration for developers. The findings provide insights for practitioners to structure unit test cases with AAA in mind, and for researchers to develop related techniques for enforcing AAA in test cases.

==> data_availability.tex <==
\section{Data Availability}
\label{sec:data_av}
Due to the double-blind rule in the review process, the data that support the findings of this study are openly available in figshare via the private link at \url{https://figshare.com/s/b1d6b70e10837aaf3f17}. Once the paper  is accepted, the data will be officially published in figshare.
For the same reason, all the refactoring tickets are replaced by the code fragment links. Once the paper is accepted, the refactoring tickets links will be added back as the references in table~\ref{tbl:issues}.
